Enabling Interactive Transcription in an Indigenous Community

We propose a novel transcription workflow which combines spoken term detection and human-in-the-loop, together with a pilot experiment. This work is grounded in an almost zero-resource scenario where only a few terms have so far been identified, involving two endangered languages. We show that in the early stages of transcription, when the available data is insufficient to train a robust ASR system, it is possible to take advantage of the transcription of a small number of isolated words in order to bootstrap the transcription of a speech collection.

==> mb-workflow-rework.tex <==
%What we are actually trying to do
In contrast to traditional approaches, we do not attempt to transcribe every word from the start of a recording, but rather we produce a sparse annotation of portions of speech, sparsely distributed throughout the speech signal.

%workflow part 1
We begin by constructing a proto-lexicon comprising acoustic parameters extracted from audio clips corresponding to real words associated with orthographic transcriptions ($w_1 , w_2 ...w_n$).
Where we have access to previous transcriptions we may simply extract segments of audio with an associated orthographic labels.
In very low resource languages, we may lack transcriptions but nevertheless have a list of words.
In this case we record words spoken in isolation via a word list elicitation app described in [x].
In both the transcription extract and word elicitation cases, we extract feature vectors from the raw signal as described in [x].
We then use spoken term detection over untranscribed audio to identify instances of each lexicon entry over the entire speech signal (see Figure 1b). %I propose getting rid of Figure 1a.
Hits are stored in the lexicon as an array of links to spans of audio (unshown).

%workflow part 2
Now we seek human confirmation of the lexicon to signal `hits'.
We achieve this with a coordinated mobile app confirmation task distributed among native speakers.
If the speaker disagrees with a signal hit then we remove the link from the lexicon to speech signal, as shown in Figure 1C.
If the speaker agrees with a signal hit then we extract the audio parameters from the signal span and add this to the lexicon, as shown in Figure 1D. 
We apply this pipeline for \textit{i} iterations with a lexicon growing each time.
The size \textit{s} of the lexicon, the \textit{n} number of words checked, the maximum
\textit{m} of extra examples for each word and the number \textit{i} of iterations are hyperparameters resulting from constraints such as the availability of recordings, speakers and manpower.

%testing here


The key idea of sparse transcription is to use spoken term detection methods to sparsely transcribe a speech collection from a limited collection of spoken words (a word list recorded in isolation or extracted directly from an existing transcription) in order to support linguists' work.
To do so, we set up a general pipeline organised as follows (see figure \ref{fig:sparse_workflow}).
We first start with a lexicon of size \textit{s} and a speech collection already transcribed with the examples used to build the lexicon (\ref{setup:0}).
The lexicon is composed by acoustic parameters extracted from audio clips corresponding to real words and their orthographic transcriptions ($w_1 , w_2 ...w_n$).
We use a spoken term detection method to retrieve words more likely to be good hits (\ref{setup:1}). A native speaker can then check which words were correctly retrieved and which were not. To test our system at this step, we simulate the human verification checking in the gold transcription.
%\laurent{A native speaker can then check on the time-aligned transcription (\ref{setup:2}) which words were correctly retrieved and which were not. This is a fast process that can be further accelerated with a dedicated interface (see section \ref{Prototype}). Such an interactive scenario is simulated in the experiments reported in the next subsections.}
%In order to simulate an human verification, we check on the time-aligned transcription to confirm if the words are correctly retrieved or not (\ref{setup:2}).
In order to have more coverage, we select the best \textit{n} per words to be verified at the next step.
We clip out from the utterances the words correctly retrieved,
we extract acoustic parameters from these clips and add them in the lexicon as extra
examples of the existing entries (\ref{setup:3}) 
%\laurent{[LB: i find that fig1d does not reflect this very well...]}. 
We allow a single word to have maximum of \textit{m} extra examples.
The wrong words retrieved are corrected (e.g. erased from the transcription) (\ref{setup:4}) and the lexicon grows with \textit{s}
new words extracted from the corpus (\ref{setup:5}).
We apply this pipeline for \textit{i} iterations with a lexicon growing each time.
The size \textit{s} of the lexicon, the \textit{n} number of words checked, the maximum
\textit{m} of extra examples for each word and the number \textit{i} of iterations are hyperparameters which can be modified according to the reality of the fieldwork.

==> workflow.tex <==
\begin{figure}[!h]
	\begin{minipage}{.35\linewidth}
		\centering
		\subfloat[]{\label{isolation}\includegraphics[width=0.7\textwidth]{coling2020/figures/isolation.png}}

		\subfloat[]{\label{recording}\includegraphics[width=\textwidth]{coling2020/figures/Roland_1.png}}
	\end{minipage}
	\hspace{3cm}
	\begin{minipage}{.35\linewidth}
		\centering
		\subfloat[]{\label{std}\includegraphics[width=0.7\textwidth]{coling2020/figures/std.png}}


		\subfloat[]{\label{verif}\includegraphics[width=0.9\textwidth]{coling2020/figures/Theo_2.png}}
	\end{minipage}
	\caption{\ref{isolation} Isolation of keywords; \ref{recording} Recording of the keywords; \ref{std} application of spoken term detection; \ref{verif} verification of the hits.}
	\label{apps}
\end{figure}
